Automated Composition of Picture-Synched Music Soundtracks for Movies

We describe the implementation of and early results from a system that automatically composes picture-synched musical soundtracks for videos and movies. We use the phrase "picture-synched" to mean that the structure of the automatically composed music is determined by visual events in the input movie, i.e. the final music is synchronised to visual events and features such as cut transitions or within-shot key-frame events. Our system combines automated video analysis and computer-generated music-composition techniques to create unique soundtracks in response to the video input, and can be thought of as an initial step in creating a computerised replacement for a human composer writing music to fit the picture-locked edit of a movie. Working only from the video information in the movie, key features are extracted from the input video, using video analysis techniques, which are then fed into a machine-learning-based music generation tool, to compose a piece of music from scratch. The resulting soundtrack is tied to video features, such as scene transition markers and scene-level energy values, and is unique to the input video. Although the system we describe here is only a preliminary proof-of-concept, user evaluations of the output of the system have been positive.

==> DBC_technical_JB.tex <==

This section briefly covers core technical concepts relevant to the implementation discussed in Section \ref{sec:implement}. 

\subsection{Music Terminology}

For brevity, we assume that the reader has a basic understanding of Western music structure, such as the way in which music is composed of a number of  \textit{bars} (or \textit{measures}), where each bar represents a segment of time containing a specified number of beats. The \textit{phrase length} is the number of bars that make up a phrase; phrases in most contemporary Western popular styles of music tend to contain four bars.

The number of beats in a bar is denoted by a piece's \textit{time signature}, for example 3/4, where the denominator indicates the duration of a beat, and the numerator indicates the number of beats in the bar. The time signature 3/4 tells us that there are 3 beats, each with the length of a quarter (1/4) note, in each bar. Similarly \textit{tempo} dictates the speed of a piece of music and is usually indicated in beats per minute (BPM). \textit{Monophonic} music is style of music that consists solely of a melody, without any harmonisation or other accompaniment. \textit{Polyphonic} music consists of two or more parts, each with its own melody, with harmonisation across parts.

\subsection{Algorithmic Composition}

%Fundamentally, musical notation is a sequence of symbols representing information that is converted into sound by a musical instrument or group of instruments. This information can be represented in a variety of formats, for example, as a score to be read by a performing musician, or as a MIDI file that can store the information digitally. Researchers have developed techniques to create statistical models of the relationships between notes in a musical sequence by analysing existing music.  Van Der Merwe and Schulze used Markov chains to model chord duration, chord progression and rhythmic progression in music \cite{5492670}. Markov chains model sequences of events as discrete states and the transition probabilities between states, and do not rely on knowledge of other states to make a transition. More sophisticated Markov models have been useful for tasks such as accompaniment or improvisation, as shown by Morris {\em et al.} \cite{morris2008exposing} in their work on human-computer interaction for musical compositions, and Sastry's 2011 thesis \cite{sastry2011n} exploring machine improvisation and composition of tabla sequences.

%Modern approaches to algorithmic composition use neural networks to tackle the problem of modelling musical compositions. Neural networks are biologically inspired computational networks that consist of neurons, or nodes, that perform simple nonlinear computations to aggregate multiple inputs into a single output. These nodes are typically connected to each other to form networks, in which the inputs to some nodes come from other nodes, that can contain multiple inter-connected layers. Nodes have a series of weighted connections to other nodes, which are determined by training the network on example patterns (in this case example sequences of music), allowing the network encode observed patterns as a connection of nodes. Neural networks are able to match the style of music they are trained on, using supervised learning to encode associations between data labels and patterns learnt by the network.

The following subsections cover the two music generation tools used in Barrington, both of which use neural-network machine learning techniques. For further details of neural networks, see e.g. \cite{Bishop95}.

\subsubsection{Magenta PolyphonyRNN}
\label{sec:poly}

PolyphonyRNN is a recurrent neural network, based on the BachBot architecture described in \cite{liang2016bachbot}. It is able to compose and complete polyphonic musical sequences using a long short-term memory (LSTM) generative model, without having to explicitly encode musical theory concepts. BachBot's success is based on modelling melodies and harmonisation independently. It is able to learn a representation of harmonisation based on samples from a corpus, and apply it to any melody. In user tests it was capable of producing music virtually indistinguishable from Bach's compositions. LSTMs differ from conventional feed-forward neural networks in that they contain feedback connections, which connect outputs from hidden layers back to the input layer of the network, allowing the network to form a representation in an iterative manner. For a more thorough exploration of the benefits of feedback neural networks see Zamir et al.\cite{zamir2017feedback}. LSTMs are discussed in more detail in \cite{HochreiterSchmidhuber1997}.



\subsubsection{IBM Watson Beat}
\label{sec:watson}

Watson Beat models polyphonic music in a similar manner to PolyphonyRNN. There is no published literature to confirm this, however, the code was released as an open-source project (\url{https://github.com/cognitive-catalyst/watson-beat/}). A brief overview of the process of developing Watson Beat is available on IBM's website \cite{IBMWatsonBeat}, in which the developers describe using supervised learning on a vast amount of data relating to each composition's pitch, rhythm, chord progression and instrumentation, as well as labeled information on emotions and musical genres. A key feature of Watson Beat is its ability to arrange the musical structure in a manner that provides the user control over individual sections of music, though it is unclear if this was manually encoded or learned from training data.

\subsection{Video Analysis}

\subsubsection{Scene Transition Detection}
\label{scene-transition-detection}

Scene transition detection, often also referred to as shot boundary detection, is a difficult task for computers, due to the variety of transition methods video editors have at their disposal. Abrupt transitions follow a predictable pattern, as the change in content from one frame to another is sudden and usually extensive. Gradual transitions often utilise visual effects to blend together two scenes into a smooth manner, such as cross-dissolves or fades, over any length of time, with very little change in content from frame to frame. This variability makes it difficult to create a single method of detecting every type of transition. Transition detection algorithms typically look at pairs of frames, computing a score for each using some defined similarity measure, then evaluating these scores against some threshold to determine if a transition has occurred.

As scene transition detection is not the focus of this project, the ability to accurately detect complex transitions is not fundamental to the outcome, therefore currently Barrington uses only two basic transition detectors, one to detect abrupt transitions ({\em cut detection}) and the other to detect fades to/from black ({\em fade detection}).

The similarity measure used for fade detection is RGB intensity. For each frame, the R, G, and B pixel values are summed to produce an intensity score. A threshold is specified such that the RGB intensity values in the majority of frames within a scene lie above said threshold; if the RGB intensity for a frame falls below the threshold, it is marked as the start of the fade, and the next frame to return above the threshold is marked as the end. This remarkably simple technique works effectively, as any fade to/from black will inevitably contain at least one black frame, which will have an RGB intensity value of 0.

Cheng et al. \cite{CHENG20012259} recommend the use of the HSI (aka HSV or HSL) 
%\footnote{Also referred to as HSV (hue, saturation, value) or HSL (hue, saturation, luminosity)} (hue, saturation, intensity)} 
colour space for computer vision tasks on colour images, as it enables segmentation in the one-dimensional hue space, which is less computationally expensive than in 3D RGB space. Cut detection requires comparing two frames for changes in content, therefore the HSI space is more appropriate than RGB. The similarity measure for cut detection is computed by taking the average of the change in hue, saturation and intensity values from one frame to the next. This aggregate value will be low for frames with little change in content, and high for frames with large changes. A threshold is then specified such that frames above the threshold are marked as abrupt transitions. 

The twin-comparison approach described in \cite{zhang1993automatic} has been adapted to combine fade and cut detection for Barrington. RGB intensity and delta HSI values are computed for each frame, and both thresholds are monitored for scene transitions.

\subsubsection{Object Detection}
\label{sec:obj}

Object detection has been the subject of intense research for many years in computer vision. Traditional machine learning approaches to object detection, such as the popular Viola-Jones method \cite{Viola01robustreal-time}, involve first defining the features of the object, then training a classifier on a labelled dataset of images containing the object. Finally, the classifier's object detection performance is evaluated at different locations and scaling factors across an image.

Convolutional neural networks (CNNs) are now considered by very many to be the preferred tool for image classification tasks. In mathematics, a convolution expresses how the shape of some function is affected as it is shifted across a \textit{static}, or non-moving, function, i.e. "blending" the two together. CNNs treat the input image as this static function and pass lots of different functions over it, each of these being a \textit{filter} that looks for a specific feature in the image. Each filter is passed over small sections of the image at a time, to build up a \textit{feature map} that tracks the locations at which various features occur across the image. 

YOLO \cite{DBLP:journals/corr/RedmonDGF15}, the method used in Barrington, utilises a single CNN for training and detection. Utilising dropouts, YOLO is able to learn a general representation for different object classes, while optimising detection performance during training, resulting in faster, more precise detection. YOLO subdivides an image into a grid, using features from across the whole image to predict the bounding box for every object class, and a confidence score that encodes the probability of that box containing an object. %Figure \ref{fig:yolo} shows an example of this in action.

%\begin{figure}[h!]
%\centering
%\includegraphics[width=\textwidth]{Diss/images/yolo.png}
%\caption[Overview of how the YOLO object detection model processes images]{YOLO subdivides the image into a grid, predicting a bounding box and confidence for objects in each grid cell, as well as the object class probability \footnotemark}
%\label{fig:yolo}
%\end{figure}

%\footnotetext{Source: \cite{DBLP:journals/corr/RedmonDGF15}}


